Text2Video: Text-driven Talking-head Video Synthesis with Personalized Phoneme-Pose Dictionary

With the advance of deep learning technology, automatic video generation from audio or text has become an emerging and promising research topic. In this paper, we present a novel approach to synthesize video from the text. The method builds a phoneme-pose dictionary and trains a generative adversarial network (GAN) to generate video from interpolated phoneme poses. Compared to audio-driven video generation algorithms, our approach has a number of advantages: 1) It only needs a fraction of the training data used by an audio-driven approach; 2) It is more flexible and not subject to vulnerability due to speaker variation; 3) It significantly reduces the preprocessing, training and inference time. We perform extensive experiments to compare the proposed method with state-of-the-art talking face generation methods on a benchmark dataset and datasets of our own. The results demonstrate the effectiveness and superiority of our approach.

==> ICASSP22 template/1-intro.tex <==
\vspace{-0.4em}
\section{Introduction}
\vspace{-0.4em}

% 1. Motivation/Application VIRTUAL CHARACTERS
% 2. Speech2video / text2video
% 3. Approach overview
% 4. Contribution 

%There are mainly two way to generate videos, one is from audio while another is from text.
%\textit{Speech2Video} is a task of synthesizing a video of human body movements from a speech audio input. The produced video should be visually natural and consistent with the given speech. 

With the advance of deep learning technology, automatic video generation from audio (\textit{speech2video}) or text (\textit{text2video}) has become an emerging and promising research topic \cite{suwajanakorn2017synthesizing,thies2019neural,liao2020speech2video}. It introduces exciting opportunities for applications such as AI news broadcasts, video synthesis, and digital humans.
\textit{Speech2Video} models are trained to map from speech to video. Because there is much speaker variability in speech, \textit{Speech2Video} models need to be trained on a large amount of data, and they are not robust to different speakers. It is also less flexible to use speech as input compared to text. Furthermore, most previous methods that generate video from speech are based on LSTM to learn audio information. However, LSTM-based methods have some limitations: 1) The network needs a lot of training data. 
2) The voice of a different person degrades output motion quality. 
3) Users can not manipulate motion output such as changing speaker attitude since the network is a black box on what is learned. 
% 3) Users can not manipulate motion output such as changing speaker attitude since the network is a black box on what is learned. 
Compared to audio-based methods, text-based methods have advantages. We here define \textit{Text2Video} as a task of synthesizing talking-head video from any text input. The video generated from a text-based method should be agnostic to the voice identity of a different person.

In this paper, we propose a novel method to generate video from text. The technique builds a phoneme-pose dictionary and trains a generative adversarial network (GAN) to generate video from interpolated phoneme poses. Forced alignment is employed to extract phonemes and their timestamps from training data to build a phoneme-pose dictionary. We applied the method to both English and Mandarin Chinese. To demonstrate the effectiveness of our approach, we conducted experiments on a number of public and private datasets. Results showed that our method achieved higher overall visual quality scores compared to state-of-the-art systems. 
%In this work, we propose a novel framework called \textit{Text2Video}. Our framework can take any text input including English and punctuation. We utilize P2FA aligner to get phoneme and their accurate timestamp from text. We build a personalized phoneme-pose dictionary of each person. Then we implement a interpolation and smoothness method to build up poses sequences. Finally, we take advantage of our modified GAN to turn poses to final output video. Besides, we extend our method to Chinese language which build phoneme-pose dictionary from pinyin.
%To demonstrate the effectiveness of our approach, we test on VidTIMIT dataset. Besides we hire 2 models, 1 American female and 1 Chinese female. We also test on youtube videos of a Chinese news broadcaster. In our experiment, we show our method get higher overall video visual quality score. Also we highlight efficiency and flexibility of our framework. 

The main contributions of this paper are summarized as follows:
1) We propose a novel pipeline of generating talking-head speech videos from any text input, including numbers and punctuation, in both English and Mandarin Chinese. The inference time is as fast as 10 frames per second.
2) We develop an automatic pose extraction method to build a phoneme - pose dictionary from any video, online or purposely recorded. With only 44 words or 20 sentences, we can build a phoneme - pose dictionary that contains all phonemes in English. 
3) To generate natural pose sequences and videos, we introduce an interpolation and smoothness method and further utilize a GAN-based video generation network to convert sequences of poses to photo-realistic videos. 


==> ICASSP22 template/2-related.tex <==
\vspace{-0.4em}
\section{Related Work}
\vspace{-0.4em}

\begin{figure}
\vspace{-0.7em}
  \centering
  \includegraphics[width=0.48\textwidth]{fig/pipeline.png}
  \caption{Pipeline of Text2Video including generating audio from text, applying forced alignment to get phoneme timestamps, searching in a phoneme-pose dictionary, applying the key pose interpolation/ smoothing module to get a sequence of poses, and generating video using modified GAN.}
  \label{fig:pipeline}
\vspace{-0.7em}
\end{figure}

\textbf{Text-Driven Video Generation.} Visual speech synthesis from text has been studied in the literature. Ezzat \cite{ezzat2000visual} introduced MikeTalk, a text-to-audiovisual speech synthesizer that converts input text into an audiovisual speech stream. Taylor~\cite{taylor2012dynamic} proposed a method for automatic redubbing of video that exploited the many-to-many mapping of phoneme sequences to lip movements modeled as dynamic visemes. 
% Text-based Video Editing is similar to our Text2Video task. 
Text-based Mouth Editing~\cite{fried2019text} is a method to overwrite an existing video with new text input. The method conducts a viseme search to find video segments with mouth movements matching the edited text. However, their synthesis approach requires a re-timed background video as input and their phoneme retrieval is agnostic to the mood in which the phoneme was spoken.

\noindent\textbf{Audio-driven video generation.} Audio-driven Video Synthesis is to drive movements of human bodies with input audio. 
% Much exciting work has been done in this area. 
For example, SythesisObama~\cite{suwajanakorn2017synthesizing} focused on synthesizing a talking-head video by driving mouth motion with speech using RNN. A mouth sequence was first generated via texture mapping and then pasted onto an existing human speech video. However, SythesisObama needs approximately 17 hours of training data for one person, which is not scalable. 
~\cite{chen2019hierarchical} utilized facial landmarks to generate video from identity image and audio signal.
~\cite{zhou2019talking} generated high-quality talking face videos using disentangled audio-visual representation.
Wang \cite{wang2020speech} proposed a GAN-based network based on the attentional multiple representations to synthesize talking-head videos from speech.
Taylor \cite{taylor2017deep} introduce a deep learning approach using sliding window regression for generating realistic speech animation. Their animation predictions are made in terms of the reference face AAM parameterization re-targeting to a character, which introduces a potential source of errors.
Ginosar \cite{ginosar2019learning} proposed a method to learn individual styles of speech gestures in two stages. However, final generated videos from their rendering stage have a few artifacts. Thies \cite{thies2019neural} developed a 3D face model by audio and rendered the output video using a technique called neural rendering ~\cite{thies2019deferred}. They proposed Audio2ExpressionNet, a temporal network architecture to map an audio stream to a 3D blend shape basis representing person-specific talking styles. 
% This method needs a long time to train. 
Previously, mouth movement synthesis is mostly deterministic: given a pronunciation, the mouth's movement or shape is similar across different persons and contexts. 
Alternately, Liao \cite{liao2020speech2video} proposed a novel two-stage pipeline of generating an audio-driven virtual speaker with full-body movements. Their method was able to add personalized gestures in the speech by interpolating key poses. They also utilized 3D skeleton constraints to guarantee that the final video is physically plausible. 
However, these method are audio-based and has limitations as mentioned earlier. 

% \textbf{Text-based Video Editing.} 
% Text-based Video Editing is similar to our Text2Video task. 
% Text-based Mouth Editing ~\cite{fried2019text} is a method to overwrite an existing video with new text input. The method conducts a viseme search to find video segments with mouth movements matching the edited text. However, their synthesis approach requires a re-timed background video as input and their phoneme retrieval is agnostic to the mood in which the phoneme was spoken.
% The selected video segments' corresponding face parameters are blended with the original sequence parameters to synthesize photo-realistic videos. 
% However, there are some limitations of the method: 1) Their synthesis approach requires a re-timed background video as input. 2) Their phoneme retrieval is agnostic to the mood in which the phoneme was spoken. 3) It requires a one hour long training sequence of the target character. 4) Testing speed is slow since the viseme search is time-consuming. 
% In addition, it cannot generate videos from any input text.

% \textbf{Text-to-speech:} 
% Text-to-speech (TTS) is to convert written text into speech. Traditional TTS \cite{Taylor2009TexttoSpeechS} has two components: a front-end text-analysis component to predict phonetic representations from text, and a back-end speech-synthesis component to generate speech from the phonetic representations by rule-based \cite{Klatt1980SoftwareFA}, parametric \cite{Tokudaetal2002}, or concatenative \cite{Hunt1996UnitSI} methods. 
% In recent years, neural TTS has tremendously improved the quality of synthetic speech \cite{Oord2016WaveNetAG,Shen2018NaturalTS,Ping2018DeepV3}. In neural TTS, the traditional hand-engineered text-analysis pipelines are replaced with learned neural text encoders. The synthetic speech is generated autoregressively at every time step. State-of-the-art neural TTS systems employ attention-based sequence-to-sequence (seq2seq) neural networks. Most of the systems generate Mel spectrogram from the text first and use a neural vocoder to synthesize waveform. 
 
% \textbf{Pose Estimation and Video Generation:} 
% Openpose~\cite{cao2018openpose} has represented the first real-time multi-person system to jointly detect human body, hand, facial, and foot keypoints on single images. 

% Vid2vid~\cite{wang2018vid2vid} learned a mapping that converts a semantic video to a photo-realistic video. In this study, the semantic label maps are image frames of the human skeleton. The core of video-to-video translation is image-to-image ~\cite{isola2017image} translation. Vid2vid has two major limitations. First, training a model needs many images of a target subject or a scene. Secondly, a learned model cannot generalize to other tasks. To apply a learned model to other targets, few-shot vid2vid~\cite{wang2019fewshotvid2vid} proposed to learn a subject-agnostic mapping that converts a semantic video and an example image to a photo-realistic video.

% \textbf{Lip-syncing:}
% Synchronization of synthesized motion with the input audio is essential. Wav2Lip \cite{prajwal2020lip} is a SOTA method in this area, which is a lip-synchronization network for
% lip-syncing random talking face videos in the wild with random speech. 



% Audio-Driven Facial Animation: These methods do not focus on photo-realistic results but on the prediction of facial motions [7,18,25,29,34]. Karras et al. [18] drive a 3D facial animation using an LSTM that maps input waveforms to the 3D vertex coordinates of a face mesh, also considering the emotional state of the person. In contrast to our method, it needs high-quality 3D reconstructions for supervised training and does not render photo-realistic output. Taylor et al. [29] use a neural network to map phonemes into the parameters of a reference face model. It is trained on data collected for only one person speaking for 8 hours. They show animations of diﬀerent synthetic avatars using deformation retargeting. VOCA [7] is an end-to-end deep neural network for speech-to-animation translation trained on multiple subjects. Similar to our approach, a low-dimensional audio embedding based on features of the DeepSpeech network [14] is used. From this embedding, VOCA regresses 3D vertices on a FLAME face model [22] conditioned on a subject label. It requires high-quality 4D scans recorded in a studio setup. Our approach works on' in the wild' videos, with a focus on temporally coherent predictions and photo-realistic renderings.






% \textbf{Human Body Pose Estimation and Fitting}  \cite{ge20193d} proposed 3d shape and pose estimation specific for hands. \cite{kanazawa2019learning, pavllo20193d} predicts 3d human motion from video or a single image, but they are limited to fit human model with limb only, not hands or face. While openpose~\cite{cao2018openpose} has been so successful at fitting the detailed human model to 2D image with all our demanded parts, including face and fingers, their output is 2D landmarks in the image space. Based on openpose, SMPL-X~\cite{SMPL-X:2019} fits a 3D skeleton to those output 2D landmarks through optimization. It also parameterizes human motion as joint angles, making it much easier to constrain joints under reasonable human articulation.  

% \noindent\textbf{Audio to Motion} \cite{karras2017audio} drives high fidelity 3D facial model using audio via end-to-end learning, where both poses and emotions are learned. \cite{shlizerman2018audio} focuses on synthesizing hand motion from music input rather than speech. Its goal is to animate graphics models of hands and arms with piano or violin music. \cite{yan2019convolutional} generates skeleton-based action using Convolutional Sequence Generation Network (CSGN). \cite{martinez2017human} instead, predict human motion using recurrent neural networks. \cite{li2017auto} uses auto-conditioned recurrent networks for extended complex human motion synthesis. They can model more complex motions, including dances or martial arts. 
% % We also adopt RNN to learn a mapping from audio to motions. However, we have a relaxed requirement on the output motion. Instead of having our output match the ground truth, we only need the result motion to be correlated to audio, as long as it looks natural and smooth.

% \noindent\textbf{Video Generation from Skeleton} 
% pix2pix~\cite{isola2017image, wang2018pix2pixHD} is a milestone in the development of GAN. It outputs a detailed real-life image from an input semantic label image. In our pipeline, the semantic label maps are image frames of the human skeleton. Nevertheless, direct applying pix2pix to an input video without temporal constraints will result in incoherent output videos. Therefore, vid2vid~\cite{wang2018vid2vid} is proposed to enforce temporal coherence between neighboring frames. 
% \cite{shysheya2019textured} proposes to render realistic video from skeleton models without building a 3D model, where the second stage of video generation is emphasized. However, it doesn't take care of facial expression and mouth movement, and it doesn't address the problem of how to generate realistic movement of the skeleton body model. \cite{cai2018deep} proposes a similar pipeline, which generates skeleton pose first and then generate the final video. However, rather than audio, its input is random noise, and its skeleton model is very simple, only having body limbs. That means its final output video lacks details on the face and fingers. 
% % In contrast, our skeleton model consists of limbs, face, and fingers. We utilize vid2vid to create final videos from the skeleton and get superior results. To obtain details on the face and hands, we modified vid2vid GAN to put more weights on these parts in the discriminator loss.

==> ICASSP22 template/3-method.tex <==
% review:
% What else are you training except for the vid2vid model? Did you retrain the Learning Gesture, Neural-voice-puppetry and Speech2Video models on your own data? It is not clear what minimum key pose distance means.... please explain it further. How do you add randomness to the output video?

% Modified:
% how were the poses extracted--is there just one pose per phoneme, or are you averaging all the phoneme-poses present in the training video? 
% Why is the real video evaluation so low? Is there some quality deterioration in the platform you used to evaluate the method? In the contributions paragraph, did you mean to say 10 frames per second? In the Figure 2 caption, did you mean to say that the output sequence is shorter? In the subjective evaluation, did you mix the identities of the speakers vs the video presenter for your method? 

\vspace{-0.4em}

\section{Method}

\vspace{-0.4em}

\begin{figure*}
   \centering
  \includegraphics[width=0.99\textwidth]{fig/smooth_interpolation_small_color2.png}
  \vspace{-0.8em}
  \caption{
%   Interpolation method. To generate the output sequence including "me" or "M IY1" in phonemes, we first find out these two key pose sequences in the phoneme-pose dictionary and the timestamps of these two phonemes in the output frames.
% %   The figure shows the case of the interval length between two phonemes is larger than the minimum key pose distance, we copy these two phoneme sequences to the output frames and 
%   The figure shows the case of the minimum key pose distance is shorter than the interval length between two phonemes. So we apply the interpolation to the middle poses between these two adjacent key poses according to our method.
Interpolation method. To generate the output sequence of ”M IY1”, we first find the key-pose sequences of "M" and "IY" in the phoneme-pose dictionary, as well as the timestamps of the two phonemes in the output. Then we copy the two key-pose sequences to the output frames and apply interpolation to the middle frames between the two adjacent key poses.
}
  \label{fig:smooth_interpolation}
  \vspace{-0.7em}

\end{figure*}

\vspace{-0.4em}

%Text2Video pipeline mainly has two parts: building a phoneme pose Dictionary from training videos and generate output videos from text input as shown in figure~\ref{fig:pipeline}.


% The procedure is illustrated in figure~\ref{fig:pipeline}.

% \subsection{Text2Video Framework}
\noindent\textbf{Text2Video Framework}. As shown in Fig.~\ref{fig:pipeline}, the input to our system is text, and the output is generated video of a talking human. Given an input text, we use TTS to generate speech from the text. Then we apply forced alignment to obtain phoneme timestamps, and lookup phoneme poses in our phoneme-pose dictionary. Next, we apply the key pose interpolation and smooth module to generate a sequence of poses. Finally, we use GAN to generate videos. 
Our method contains two key components: building a phoneme-pose dictionary from training data (audio and video of speech) and training a model to generate video from phoneme poses. 

%\textbf{Speech to text}. There are %some useful tools to get timestamp %rom audio, such as google cloud %Speech-to-Text API. Speech-to-Text can %include timestamp values in the %response text. Timestamp values show %the beginning and end of each word %that is recognized in the audio. A %Timestamp value represents the amount %of the time from the beginning of the %audio. 

%However, getting words timestamp is %not good enough since languages like %English is composed with phonemes. So %we divide not only sentences to words, %but also words to phonemes. 

%Phonemes are the basic units of the %sound structure of a language. They %are produced with different
%positions of the tongue and lips, for %example, with lips rounded (e.g. /u/) %or spread (e.g. /i/), or wide-open %(e.g., /a/) or closed (e.g., /m/). 

% \subsection{Build Phoneme-Pose Dictionary}
\noindent\textbf{Phoneme-Pose Dictionary}.
Phonemes are the basic units of the sound structure of a language. They are produced with different positions of the tongue and lips, for example, with lips rounded (e.g. /u/) or spread (e.g. /i/), or wide open (e.g., /a/) or closed (e.g., /m/). English has 40 phonemes if we don't count lexical stress. 
% The phonemes are listed in supplemental materials appendix Fig. ~\ref{fig:ARPABET}
%Appendix 1. 
There are three levels of lexical stress in English: primary stress, secondary stress, and unstress. Stress may influence the position of the lips in speech production. For example, the vowel 'er' in the word \textit{permit} is stressed when the word is a noun and is unstressed when it is a verb. The mouth is slightly more open when pronouncing the stressed 'er'. Therefore, we distinguish stress in the English phoneme-pose dictionary. For Mandarin Chinese, we use initials and finals as the basic units in the phoneme-pose dictionary. This is because phonemes in the finals in Chinese are more blended and don't have a clear boundary between each other \cite{ren1986}. 
% Appendix Fig. ~\ref{fig:pinyin} is a list of Mandarin initials and finals. 
We build a phoneme-pose dictionary for English and Mandarin Chinese, respectively, mapping from phonemes to lip postures extracted from a speech production video.

\noindent\textbf{Key Pose Extraction}. First, we use Openpose~\cite{cao2018openpose} to extract key poses from training videos by averaging all the phoneme-poses present in the training video. Then we build up the phoneme-pose dictionary from our phoneme extraction pipeline described below.

\noindent\textbf{Phoneme Extraction}.
We employed the P2FA aligner \cite{yuan&liberman2008} to determine phonemes and their time positions in an utterance. The task requires two inputs: audio and word transcriptions. The transcribed words are mapped into a phone sequence in advance using a pronouncing dictionary or grapheme to phoneme rules. Phone boundaries are determined by comparing the observed speech signal and pre-trained, Hidden Markov Model (HMM) based acoustic models. In forced alignment, the speech signal is analyzed as a successive set of frames (e.g., every 10 ms). The alignment of frames with phonemes is determined by finding the most likely sequence of hidden states (which are constrained by the known sequence of phonemes derived from transcription) given the observed data and the acoustic models represented by the HMMs. 
% The procedure is illustrated in Figure~\ref{fig:alignment}. 
% The video was captured at 25fps. 
Then, we store a sequence of poses for each phoneme in the dictionary based on the alignment. The width of the phoneme-poses is determined based on the dataset video frame rate and average speaking rate.
% The width of the phoneme-poses was set to 7 frames for VidTIMIT dataset(which was determined based on the video frame rate and average speaking rate), i.e., every phoneme in the phoneme-pose dictionary has a sequence of 7 frames of poses.
% Our video is captured at 25 fps. Phoneme poses width depends on video frame rate and average speaker rate. We set phoneme poses width equals to 7 frames for the VidTIMIT dataset which means for each phoneme we extract 7 frames pose sequences in the phoneme pose dictionary. 


% \begin{figure*}
%   \centering
%   \includegraphics[width=0.85\textwidth]{fig/forced alignment.png}
%   \caption{Forced alignment of our system. The boundaries of the phonemes in the word "this" are determined through forced alignment of acoustic frames and pre-trained acoustic models. "this" has three pronunciations in the dictionary; the alignment selects a pronunciation that best matches the acoustic signal, which is "DH", "IH", "s". The aligner also outputs timestamps of these three phonemes.}
%   \label{fig:alignment}
% \end{figure*}

% \subsection{Text to Speech}
\noindent\textbf{Text to Speech}.
We use Baidu TTS to generate audio from text input. The system's default female and male voices are used. For personalized video generation, one can use any technique to generate a voice of his/her own choice. The voice of a different person will not affect the generated video quality of our method.

% \subsection{Key Pose Insertion}
\noindent\textbf{Key Pose Insertion}.
To generate a sequence of poses, we need to do key pose insertion for the missing poses between key poses. We go through all phonemes one by one in speech and find their corresponding poses in the phoneme-pose dictionary. 
% A phoneme pose is inserted into a timestamp with a ramp length number of frames before and after its insertion time point. The ramp length depends on the video frame rate and ramp duration.
When we insert a pose into a video, an interpolation is performed in their pose parameter space. We determine the interpolation strategies by taking consideration of the following factors:
% motion width 
phoneme poses width (which represents the number of frames for a key pose sequence extracted from the phoneme-pose dictionary), and minimum key poses distance (which determine if we need to do interpolation). Minimum key poses distance between two phonemes equals to the sum of (half of the first phoneme pose width + half of the second phoneme pose width). The equation is defined as:

\vspace{-0.4em}

\begin{equation}
    distance=\frac{1}{2} \times width_{i} + \frac{1}{2} \times width_{i+1},
\end{equation}
\vspace{-0.4em}

where $distance$ is minimum key poses distance and $width$ is phoneme pose width. 
Our interpolation strategies is:
If the interval length between two phoneme key pose frames is larger than or equal to the minimum key pose distance, we will do interpolation using the key pose\textsubscript{i} and key pose\textsubscript{i+1}. If the interval length between two phoneme key pose frames is smaller than the minimum key pose distance, we will skip the key pose\textsubscript{i+1} and using the key pose\textsubscript{i} and key pose\textsubscript{i+2} to do interpolation. 
% The rest-frame will be the idle frame when the speaker does not speak. 
% If interval length equals minimum key pose distance, we will copy the phoneme pose to the output sequence of poses.
% If the interval length between two phonemes is smaller than the minimum key pose distance, 
Then, we blend key poses between two key pose sequences with a weighted sum of phoneme poses using the method showed in Fig.~\ref{fig:smooth_interpolation}. The new frames in the output sequence are interpolated between two key pose frames, weighted by their distance to those two frames. Weight is inverse proportional to the distance from a key frame which means the larger the distance, the smaller the weight.
% Weight will be the distance to one key pose divide by the interval length of two keyframes.

% \subsection{Smoothing}
\noindent\textbf{Smoothing}.
Smoothing is implemented after the interpolation step.   
The phoneme pose is directly copied to its time point within the video. The smoothing of the motion of poses is controlled by a smooth width parameter.
% To make human motion more stable, we smooth all 68 face keypoints except the mouth part based on openpose which is shown in figure~\ref{fig:keypoints_face}.
To make human motion more stable, we smooth all face keypoints except the mouth part. Because smoothing the mouth directly will sacrifice the accuracy of the mouth shape corresponding to phonemes, we calculate the mouth center and shift for all mouth key points corresponding to the center of the mouth. The new frames are linearly interpolated, weighted by their distance to other frames in the sliding window. Finally, we copy mouth key points to the mouth center of each frame. We smooth the frames one by one in the sliding window till the end of a pose sequence.  

% If the interval length between two phoneme key pose frames is larger than the minimum key pose distance, we will add the rest frames.

% Else if the interval between two phonemes is smaller than the length of (2 * motion width + transition width), we will reduce the ramp length to a shorter interval length. 

% Otherwise, we will apply the interpolation method as mentioned above with a weighted sum of phoneme poses.

% Right after we finish the interpolation step, we begin the smoothing step.   
% The phoneme pose is directly copied to its time point within the video. The smoothing of the motion of poses is controlled by a smooth width parameter. Here we set smooth width to 4 in our experiments for the VidTIMIT dataset. We replace frames from the start frame to a key pose on both sides. The new frames are linear interpolated between ramp start frame and key pose frame, weighted by their distance to those 2 frames.

% replace frames from the ramp start point to the key pose frame on both sides. The new frames are interpolated between the ramp start frame and key pose frame, weighted by their distance to those two frames. 

% \subsection{Train Video Generation Network}
\noindent\textbf{Training Video Generation Network}.
We utilize the generative network vid2vid ~\cite{wang2018vid2vid} to convert our pose sequences into real human speech videos. We modified the GAN network to put more weights on the face part. 

==> ICASSP22 template/4-exp.tex <==
\vspace{-0.4em}
\section{Experiments}
\vspace{-0.4em}

% \subsection{Dataset and Settings}
% \noindent\textbf{Text to Speech}.

\noindent\textbf{Datasets}. To validate our approach, we used the VidTIMIT dataset \cite{sanderson2009multi}. The VidTIMIT dataset consists of video and corresponding audio recordings of 43 people (19 female and 24 male), reading sentences chosen from the TIMIT corpus \cite{Garofolo1992}. There are ten sentences for each person. The sentences' mean duration is 4.25 seconds, or about 106 video frames (25 fps).
To test our algorithm, we also recorded a dataset of our own. We invited a female native English speaker to do recording via zoom meeting. 
% We captured the video from a zoom meeting with the subject, and the resolution is 448*512. 
We prepared prompts, including 44 words and 20 sentences. 
% The word examples are transcribed in ARPABET ~\ref{fig:ARPABET}.
We also tested our algorithm in other languages like Mandarin Chinese. We used a native Mandarin Chinese speaker (female) as a model and captured a video of her reading a list of 386 syllables in Pinyin. The total recorded video is approximately 8 mins. 
Besides, we used online Youtube videos of a Chinese news broadcaster to test our algorithm. 
% Details of the four datasets are compared in table~\ref{tab:dataset}. 

% \noindent\textbf{Implementation Details.} 
% In our experiments, the video frame rate is 25 fps. We set phoneme poses width equals to 7,
% % motion width to 3, 
% % transition width to 5, 
% minimum key pose distance to 4, and smooth sliding window size to 9. Fig. ~\ref{fig:VidTIMIT_result} shows VidTIMIT output. 
% The result videos are in the supplementary multimedia file and the demo video is at \url{https://youtu.be/d5MFzHxeOTs}.


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \begin{table*}[]
% \centering

% \caption{Dataset detail of VidTIMIT, data from two models we hired and Youtube. Dataset details include training video duration, data source, recording resolution, and how a phoneme-pose dictionary was built from the data.}
% \label{tab:dataset}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lllll@{}}
% \toprule
%                     & Training video time & Captured by/ Data From & Video Resolution & Phoneme-pose dictionary built from \\ \midrule
% VidTIMIT dataset    & 1 min per person,  43 people  & Digital camera         & 512*384              & 10 English sentences                       \\
% American Female     & Total 6 min.  & Zoom           & 640*480   & 44 English words                    \\
% Chinese Female      & Total 8 min.  & Digital camera & 1920*1080 & 386 Chinese pinyin                  \\
% Chinese Male        & Total 10 min. & Youtube        & 512*448   & Chinese pinyin extracted from video \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}


% \subsection{Evaluation}
\noindent\textbf{Evaluation}.
To evaluate the generated videos' quality, we conducted a human subjective test on Amazon Mechanical Turk (AMT) with 401 participants. We showed a total of 5 videos to the participants in which the identities of the speakers and the video presenter are mixed. The participants were required to rate those videos' quality on a Likert scale from 1 (very bad) to 5 (very good). The ratings include 1) The face in the video is clear; 2) The face motion in the video looks natural and smooth; 3) The audio-visual alignment (lip-sync) quality; 4) The overall visual quality of the video. We compared our results with SoTA approaches, including LearningGesture~\cite{ginosar2019learning}, neural-voice-puppetry~\cite{thies2019neural}, and Speech2Video~\cite{liao2020speech2video}. Since these three methods are audio-based and use the real human voice in their demo videos. We also used a real human voice for the comparison. Table~\ref{tab:score} shows the scores from the user study for all methods. Our method has the best overall quality score compared to the other 3 SOTA methods. Besides, our text-based method is more flexible than the aforementioned audio-based method and not subject to vulnerability due to speaker variation.

\begin{table}[]
\centering
\begin{tabular}{lllll}
\hline
                         & Q1    & Q2    & Q3    & Q4    \\ \hline
LearningGesture          & 3.424 & 3.267 & 3.544 & 3.204 \\
Neural-voice-puppetry    & 3.585 & 3.521 & 3.214 & 3.465 \\
Speech2Video             & 3.513 & 3.308 & 3.094 & 3.262 \\
% Our method (TTS)         & 3.623 & 3.592 & 3.105 & 3.387 \\
\textbf{Text2Video}      & \textbf{3.761} & \textbf{3.924} & \textbf{3.567} & \textbf{3.848} \\
\hline
\end{tabular}
\caption{User Study. Average scores of 401 participants on 4 questions. 
Q1: face is clear. Q2: The face motion in the video looks natural and smooth. Q3: The audio-visual alignment (lip sync) quality. Q4: Overall visual quality.
}
\label{tab:score}
\vspace{-0.3em}
\end{table}


% \subsection{Ablation Study}

\begin{table}[]
% \hfill
% \parbox{.45\linewidth}{
\centering
\begin{tabular}{@{}llllll@{}}
\toprule
                              & Q1   & Q2   & Q3   & Q4     \\ \midrule
% Text2Video(w/TTS)             & 3.33 & 3.51 & 3.23 & 3.09  \\
% Text2Video(w/Human voice)     & 3.28 & 3.50 & 3.21 & 3.18  \\
% Real video                    & 3.52 & 3.87 & 3.86 & 3.46  \\ \bottomrule
Text2Video(w/TTS)             & 3.73 & 3.91 & 3.63 & 3.55  \\
Text2Video(w/Human voice)     & 3.78 & 4.01 & 3.71 & 3.68  \\
Real video                    & 4.02 & 4.47 & 4.46 & 4.06  \\ \bottomrule
\end{tabular}
\caption{Ablation study on different voice quality. Average scores of 401 participants on same questions as Table 2. 
% Q1: face is clear. Q2: The face motion in the video looks natural and smooth. Q3: The audio-visual alignment (lip sync) quality. Q4: Overall visual quality.
}
\label{tab:video_score}
\vspace{-0.6em}
\end{table}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.47 \textwidth]{fig/output_results2.png}
%   \caption{Output results of our method. From left to right are result from VidTIMIT dataset, American Female, Chinese Female, Chinese Male. The result demos can be found in the supplementary video.}
%   \label{fig:result}
% \end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.49 \textwidth]{fig/fadg0_output.png}
  \caption{The output of our method from the VidTIMIT dataset. The first line shows the ground truth video clips of ``She" or ``SH IY1" in phonemes, the second line shows the output pose sequences, and the third line shows the synthesized image sequences generate from pose sequences. The result videos are at \url{https://tinyurl.com/9kfr8du2}. }
  \label{fig:VidTIMIT_result}
  \vspace{-0.6em}
\end{figure}

\noindent\textbf{Ablation Study}.
We also implemented the following user study to validate the effectiveness of our method. We showed three videos to the participants: one real and two synthesized. We used the transcription of speech in the real video to generate two synthesized videos, one with the real voice and the other with a TTS voice, to compare with the real video. We played the videos in a random order without telling the participants which one is real. As shown in Table~\ref{tab:video_score}, our output video with human voice got 3.68, and the real video got 4.06 (out of 5) on overall visual quality. The generated video is 90.6\% of the overall quality of the real video. In particular, our proposed method has similar performance on face clarity and motion smoothness compared to the real video. The video with a TTS voice got 87.4\% of the overall quality of the real video. The difference should come from the quality of the TTS audio. We simply picked an average female voice in the experiment. Using a better TTS or using a learning method to train a personalized human voice could improve the overall audio quality. Based on the user study, the overall visual quality from our text-based video generation method is barely correlated with the voice quality.
% which prove the advantage over audio-based method. 

% \subsection{Ablation Study}
% First, we perform ablation studies of phonetic dictionaries with lexical stress. We perform the study in a self-reenactment scenario in which we compare our result to the input frames. We compare our complete approach with lexical stress with simplified approaches without lexical stress. 


% Then, we perform ablation studies of state aligner. 

% In the acoustic models used for forced alignment, every phoneme has three hidden states to model the beginning, the middle, and the end part of a phone.



% First, we perform word alignment compared with phoneme alignment.


% \subsection{Self Reenactment}


% \subsection{Running Times and Hardware}
\noindent\textbf{Running Times and Hardware}.
We compare our method with SythesisObama~\cite{suwajanakorn2017synthesizing}, neural-voice-puppetry~\cite{thies2019neural}, and Speech2Video~\cite{liao2020speech2video} on training data size, data preprocessing and training time, and inference time. 
Our method needs the least amount of data to train a model. Using our fine-grained 40 words or 20 sentence list to capture all phonemes in English, the training video input can be less than 1 minute. 
% Using existing videos to extract a phoneme-pose dictionary will also make the training data a similar size. 
% The total number of images we need to train is 1250 images for 25 fps 60s video.
Besides, our method needs the least preprocessing and training time among all four approaches. 
Preprocessing time of our approach includes running Openpose and building up a phoneme-pose dictionary. 
% The training time of our method is relatively short. 
For the VidTIMIT dataset 
% which has a resolution of 512*384
, it took about 4 hours to train our modified vid2vid GAN on Nvidia M40 GPUs while other methods need at least 30 hours. 
% , a model trained on 15 epochs is good for inference. 
The inference time of our method is around 0.1 second per frame, which is similar to Neural-voice-puppetry but much faster than SythesisObama (1.5 s/frame) and Speech2Video (0.5 s/frame) on Nvidia 1080Ti. 
% Details of comparison can be found in appendix Table \ref{tab:time}. 
% The video generation rate is around 10 fps on a single NVIDIA GTX 1080 GPU. 

\vspace{-0.3em}


==> ICASSP22 template/5-con.tex <==
\vspace{-0.4em}
\section{Conclusion}
% \section{Conclusion and Future Work}
\vspace{-0.4em}

In this paper, we proposed a novel method to synthesize talking-head video from any text input. Our method includes an automatic pose extraction to build a phoneme - pose dictionary from any video. Compared to SOTA audio-driven methods, our text-based video synthesis method needs significantly less training data and has 10 times faster preprocessing and training time. We demonstrated the effectiveness of our approach for both English and Mandarin Chinese text inputs. 
% In the future, we will extend our method to other languages. 

% We will also integrate voice learning methods into our training pipeline to generate personalized voices. 




